The Sticky Path to Expressive Querying: Decidability of Navigational Queries under Existential Rules

Extensive research in the field of ontology-based query answering has led to the identification of numerous fragments of existential rules (also known as tuple-generating dependencies) that exhibit decidable answering of atomic and conjunctive queries. Motivated by the increased theoretical and practical interest in navigational queries, this paper considers the question for which of these fragments decidability of querying extends to regular path queries (RPQs). In fact, decidability of RPQs has recently been shown to generally hold for the comprehensive family of all fragments that come with the guarantee of universal models being reasonably well-shaped (that is, being of finite cliquewidth). Yet, for the second major family of fragments, known as finite unification sets (short: fus), which are based on first-order-rewritability, corresponding results have been largely elusive so far. We complete the picture by showing that RPQ answering over arbitrary fus rulesets is undecidable. On the positive side, we establish that the problem is decidable for the prominent fus subclass of sticky rulesets, with the caveat that a very mild extension of the RPQ formalism turns the problem undecidable again.

==> x4-sticky-decidable.tex <==

\section{Decidablility of regular path queries over sticky rulesets}

In the next section we are going to show the proof of the following:

\begin{theorem}\label{thm:sticky-main}
RPQ entailment under sticky rulesets is decidable.
\end{theorem}


To simplify the quite involved proof of the above we restrict the query language to RPQs. However, it is straightforward to obtain the following as a consequence:

\begin{theorem}\label{thm:extended-sticky-main}
2RPQ entailment under sticky rulesets is decidable.
\end{theorem}

One can obtain \cref{thm:extended-sticky-main} by a simple reduction. Take a sticky ruleset $\rs$ over signature $\sig$, a database $\db$ and a 2RPQ $\rpq$. Keep $\db$ intact, add a single rule 
    ${\epred(x,y)}\to{{\epred'}(y,x)}$
to $\rs$ for every binary predicate $\epred \in \sig$, and replace every occurence of inverted symbol $\inv{\epred}$ with \rebut{$\epred'$} in the regular expression of $\rpq$. 
%
It should be clear that entailment questions for original and transformed problems are equivalent. Finally, note that the transformation preserves stickiness of the ruleset. 


%\section{Proof of Theorem~\ref{thm:sticky-main}}\label{sec:sticky-main-proof}

The rest of the section is dedicated to the proof of \Cref{thm:sticky-main}. 
Fix, until the end of this section, a database $\db$, a sticky ruleset $\rs$.
%and a RPQ $\rpq$. 
We show decidability through two semi-decision procedures.

\rebut{
\noindent
\textbf{On repeated free variables of RPQs.} We would like to note that, by definition, we do not support RPQs of the form $A(x,x)$ and $\exists{x}.A(x,x)$. It appears to us that handling any "variable joining" requires a very distinct set of techniques. Therefore, we feel that those two cases should naturally fall under class of \emph{conjunctive} (2)RPQs. This should become apparent in the following section.}

\subsection{Recursive Enumerability}
This part \rebut{follows standard technique appealing to recursive enumerability of consequences of FO theories}.

\begin{observation}
Given a Boolean RPQ $Q = \Exists{x,y} A(x,y)$ one can write a Datalog rule set $\rs_Q$ with one distinguished nullary predicate \textsc{Goal}, such that for every instance \rebut{$\db$}:
$$\database,\; \ruleset \models Q \quad\iff\quad \database,\; \rebut{\ruleset \,\cup\,} \rs_Q \models \textsc{Goal}.$$ 
\end{observation}
\begin{proof}
Let $\autom$ be any DFA with its regular language being the same as the language of $A$. For every state $q_i$ of $\autom$ let $\qpred_i$ be a \rebut{fresh} and corresponding \rebut{unary} relational symbol. Then the Datalog rule set $\rs_Q$ contains the following rules:
\begin{align*}
\adrule{}{\qpred_{0}(x)} \tag{for the starting state $q_0$}\\
\adrule{\qpred_{i}(x), \epred(x,y)}{\qpred_{j}(y)} \tag{if $\pair{q_i, \epred} \mapsto q_j$ is in $\autom$}\\
\adrule{\qpred_{f}(x)}{\textsc{Goal}}\tag{for the accepting state $q_f$}
\end{align*}
%
In essence, the chase of any instance and the above ruleset will have every domain element annotated with the states in which they can be reached by a walking automaton starting from some other domain element.
\end{proof}

From this, as $\db \wedge \rs \wedge \rs_{\rpq}$ is an FO theory, we can semi-decide $\db, \rs \cup \rs_{\rpq} \models \textsc{Goal}$. Thus, we can semi-decide $\db, \rs \models \rpq$ as well.


\subsection{Co-recursive Enumerability}
This part is much harder than the above and requiring a fresh approach. 
In essence, the co-procedure exploits the fact that, after a certain pre-processing of $\db$ and $\rs$, non-entailment of \rebut{any} $\rpq$ is witnessed by a finite instance.

\begin{definition}\label{def:finite-controllability}
Given a query language $\mathfrak{L}$ and a ruleset $\rs$ we say that $\rs$ is {\em finitely $\mathfrak{L}$-controllable} \iffi for every $Q \in \mathfrak{L}$ and for every database $\db$ such that $\db, \rs \not\models Q$ there exists a finite model $\mathcal{M}$ of $\db$ and $\rs$ such that $\mathcal{M} \not\models Q$.
\end{definition} 

\begin{lemma}\label{lem:sticky-co-semi-decision}
One can compute a database $\dbp$ and a ruleset $\rsp$ such that $\rsp$ is finitely RPQ-controllable \rebut{and such that for every Boolean RPQ $\rpq$ we have}  $\db, \rs \models \rpq \;\iff\; \dbp, \rsp \models \rpq$.
\end{lemma}

In view of this lemma, we can ``co-semidecide'' $\db, \rs \models \rpq$ (that is, semi-decide $\db, \rs \not\models \rpq$) 
by enumerating all finite instances and terminating whenever a $\rpq$-countermodel of $\dbp, \rsp$ is found.

\subsection{The proof of \cref{lem:sticky-co-semi-decision}}



Before we start with formalities, we make a small assertion regarding input rulesets and databases. It makes the latter part easier, and could be achieved by taking equivalent but cosmetically transformed databases, rulesets, and RPQs instead of the provided ones.
\begin{assertion}\label{as:no-intra-atom-joins}
Every database and ruleset contains no atom with repeated terms.
\end{assertion} 
We defer the precise definition of such transformation to the \cref{app:transformation} and below we present a high-level overview.
We preprocess $\db$ and $\rs$ by annotating their atoms. For example, $\epred(a, b, b, c)$ becomes $\epred_{1,2,2,3}(a,b,c)$. Rulesets have to be expanded by taking every potential equivalence relation on body variables into account while applying the same transformation to their heads. For example:
\orange{
\begin{equation*}
\narule{\epred(x,y)}{z}{\rpred(x, y, z, z)}\tag*{is expanded into:}
\end{equation*}
\begin{align*}
\arule{\epred_{1,2}(x,y)}{z}{\rpred_{1,2,3,3}(x, y, z)},\\ \arule{\epred_{1,1}(x)}{z}{\rpred_{1,1,2,2}(x,z)}
\end{align*}
}
The last thing necessary to consider is the treatment of binary loops $\epred(t,t)$ --- now turned into unary atoms $\epred_{1,1}(t)$ --- by any given RPQ. 
To not overcomplicate the consideration, we presume that RPQs are, in fact, able to ``see'' atoms of the form $A_{1,1}(t)$ and treat them as if they were binary atoms in the original form, i.e., $A(t,t)$.
%To not multiply entities beyond necessity, our RPQs are simply allowed to read such created unary atoms $\apred_{1,1}(t)$ as $\apred(t,t)$.

The above assertion is meant to avoid adding yet another layer of transformations to the already complicated proof that follows. It is straightforward to verify that various ruleset-surgeries  performed after this point do not invalidate the above assertion in the slightest. 

\subsection*{From $\db$ to $\dbp$}

\begin{definition}
Let $\dbp = \chase{\db, \rs}|_{\adom{\db}}$
\end{definition}

\noindent
That is, $\dbp$ is $\db$ \rebut{``saturated''} under $\rs$. Of course we can compute $\dbp$:

\orange{
\begin{observation}\label{obs:db-and-dbp-are-equivalent}
$\dbp$ is computable and $\chase{\db, \rs} = \chase{\dbp, \rs}$
\end{observation}
\begin{proof}
As $\rs$ is \fus we can rewrite each atomic query and ask if it holds for any tuple of constants of $\db$.
%
\rebut{The second part follows from:} $\chase{\db, \rs} \subseteq \chase{\dbp, \rs} \subseteq \chase{\chase{\db, \rs}, \rs}$ and $\chase{\db, \rs} = \chase{\chase{\db, \rs}, \rs}$.
\end{proof}
}
\begin{comment}
\begin{observation}
$\chase{\db, \rs} = \chase{\dbp, \rs}$
\end{observation}
\begin{proof}
Note that $\chase{\db, \rs} \subseteq \chase{\dbp, \rs} \subseteq \chase{\chase{\db, \rs}, \rs}$ and $\chase{\db, \rs} = \chase{\chase{\db, \rs}, \rs}$.
\end{proof}
\end{comment}

\subsection*{From $\rs$ to $\rsp$ -- Preparation}

In this section, we heavily rely on both the stickiness of $\rs$ and its rewritability.\footnote{Recall that every sticky ruleset is \fus.}  The below relies on the idea that for the \fus rulesets, rewriting can be also applied to bodies of rules -- yielding a new equivalent ruleset. This transformation preserves stickiness of the input ruleset (\cref{lem:rsa-is-sticky}) and, importantly, it preserves Boolean RPQ entailment when an adjusted database is used (\cref{lem:rsa-good-entailment}).
Some of the heavily technical arguments are deferred to the appendix.

\newcommand{\rewop}{\mathtt{rew}}
\newcommand{\rrew}{\rew(\rs)}
\newcommand{\rhorew}{\rew(\rho, \rs)}
\begin{definition}\label{def:body-rewriting}
For a rule $\rho \in \rs$ of the form:~$\cnarule{\alpha(\vx, \vy)}{\vz}{\beta(\vy, \vz)}$
let $\rhorew$ be the following set of existential rules:
\begin{align*}
    &\set{\narule{\gamma(\vx', \vy)}{\vz}{\beta(\vy, \vz) \mid \\ &(\Exists{\vx'}\gamma(\vx', \vy)) \;\in\; \rew(\Exists{\vx} \alpha(\vx, \vy), \rs)}}.
\end{align*} 
%
Finally, let $$\rrew= \rs \cup \bigcup_{\rho \in \rs}\; \rhorew.$$
\end{definition}


\begin{lemma}\label{obs:rewriting-preserves-skicky}
The ruleset $\rrew$ is sticky.
\end{lemma}
\begin{proof}
\rebut{Can be found in} \cref{sec:rewriting-preserves-skicky}.
\begin{comment}
We shall use the rewriting procedure of König et al. \cite{existential-rules-rewriting-procedure-montpelier} (Algorithm 1) as the foundation for our reasoning. For the sake of completenes we include a verbatim copy of therein presented algorithm:

\begin{figure}[H]
\centering
\includegraphics[width=0.6\textwidth]{figures/rewriting_alg.png}
\caption{The rewriting algorithm presented in work of König et al. \cite{existential-rules-rewriting-procedure-montpelier}}.
\end{figure}

In our case the rewriting operator $\mathtt{rew}$, thanks to \cref{as:no-intra-atom-joins}, degenerates significantly. Consider the following definition:

Given a CQ $Q$ a rule $\rho = \narule{\alpha(\vx, \vy)}{\vz}{\beta(\vy, \vz)}$ and a homomorphism $h$ from the head of $\rho$ to $Q$ we say that $\rho$ is {\em backward applicable} to $Q$ w.r.t. $h$ if and only if 
\begin{enumerate}
	\item $h(\beta(\vy, \vz))$ is the only atom of $Q$ containing terms of $h(\vz)$.
	\item $h(\vz)$ consists of existentially quantified variables only.
\end{enumerate}
We denote the conjunction of the two formulae above as $\mathbf{back}(Q,\rho,h)$. Now, assuming that $\mathbf{back}(Q,\rho,h)$ holds we denote with $\mathtt{rew}(Q, \rho, h)$ the following CQ:
$$Q \setminus h(\beta(\vy, \vz)) \cup \alpha(\vx', h(\vy))$$
where $\vx'$ is a tuple of fresh variables. Then $\mathtt{rew}(Q, \rs)$ is defined as follows:
$$\mathtt{rew}(Q, \rs) = \set{\mathtt{rew}(Q, \rho, h) \mid \Exists{\rho, h} \mathbf{back}(Q, \rho, h)}.$$

Given any sticky ruleset $\rs'$ and its rule $\rho$ let $\rewop(\rho, \rs')$ denote the following ruleset
$$\rs' \cup \set{\narule{\gamma(\vx', \vy)}{\vz}{\beta(\vy, \vz) \;\mid\; (\Exists{\vx'}\gamma(\vx', \vy)) \in \rewop(\Exists{\vx} \alpha(\vx, \vy), \rs)}}$$ 
It is trivial to note that $\rs' \cup \rewop(\rho, \rs')$ is sticky as well. Then the observation follows, by a simple inductive reasoning, from soundnes and completenes of the above Algorithm 1.
\end{comment}
\end{proof}



\begin{definition}\label{def:rnf}
Let $\rnf$ be $\set{\core(\rho) \mid \rho \in \rrew}$.
\end{definition}


\begin{lemma}\label{cor:about-rnf}
For every Boolean RPQ $\rpq$ we have: $$\chase{\db, \rs} \models \rpq \iff \chase{\dbp, \rnf} \models \rpq.$$
\end{lemma}
\begin{proof}
    Can be found in \cref{app:cor:about-rnf}
\end{proof}

\begin{lemma}\label{cor:cleanup}
Let $\rs'$ be the subset of $\rnf$ that consists of all its Datalog rules containing only predicates of arity two and having at least two distinct join variables. Then:
$$\chase{\dbp, \rnf} = \chase{\dbp, \rnf \setminus \rs'}.$$
\end{lemma}
\begin{proof}
\rebut{Can be found in \cref{app:cor:cleanup}}
\begin{comment}
It should be clear that $\chase{\dbp, \rnf \setminus \rs'} \subseteq\\ \chase{\dbp, \rnf}.$
%
Assume toward a contradiction that there exists a binary atom in $\chase{\dbp, \rnf}$ but not in $\chase{\dbp, \rnf \setminus \rs'}$. Let $\alpha$ be one of the earliest such atoms. Let $t$ and $t'$ be terms of $\alpha$ and $i$ be the smallest natural number such that both $t$ and $t'$ appear in the $i$th chase step and assume w.l.o.g. that $t'$ has been added last. \rebut{From quickness of $\rnf$ (\cref{obs:prop-of-rnf})}, we know that there is a trigger $\pi = \pair{\rho, h}$ such that $\pi(\step{i - 1}{\dbp, \rnf}) = \alpha$. Of course, $\rho \in \rs'$ thus it is a Datalog rule that has a binary atom in its head. Moreover, in $\rho$, as it is sticky, every join variable has to be its frontier variable. From this and the assumption we conclude that $\rho$ has in its body exactly two join variables. Let $x$ and $y$ be the frontier variables of $\rho$ and $h(x) = t$. As the rule $\rho$ is cored (see \cref{def:cored-rule}), and as $t'$ has only just appeared in the chase -- meaning that there is only one single atom containing $t'$ -- it follows that $y$ could not be a join variable in $\rho$ - \rebut{a contradiction}.
\end{comment}
\end{proof}

Note that the above might be a bit counter-intuitive as it seems we remove important bits of the ruleset. To some degree it is the case, as given any database $\db'$ it might not be true that $\chase{\db', \rnf} = \chase{\db', \rnf \setminus \rs'}$. \rebut{However, the crucial aspect is that we focus solely on $\dbp$, which is already saturated in Datalog.}
%The trick, however, is that we care only about $\dbp$ - which is already Datalog-saturated. 

\newcommand{\rsa}{\rs_\mathrm{pruned}}
\newcommand{\rsjl}{\rs_\mathrm{joinless}}
\newcommand{\rsst}{\rs_\mathrm{sticky}}
\newcommand{\rsste}{\rs_\mathrm{sticky}^{\exists}}

\begin{definition}\label{def:rsa}
    Let $\rsa$ denote $\rnf \setminus \rs'$, let $\rsjl$ be the joinless subset of $\rsa$ and let $\rsst$ be its remainder.

\end{definition}
\subsubsection*{Results of the preparation}
While the above can be challenging at times to fully grasp, the results of the preparatory section can be confined to the two following lemmas. The first one, guarantees that the ruleset-surgeries preserve Boolean RPQ entailment as long as $\dbp$ is used instead of $\db$. The second, shows that $\rsa$ is still sticky.

\begin{lemma}\label{lem:rsa-good-entailment}
    For every Boolean RPQ $\rpq$ we have:
    $$\chase{\db, \rs} \models \rpq \iff \chase{\dbp, \rsa} \models \rpq.$$
\end{lemma}
\begin{proof}
    Directly from \cref{cor:about-rnf,cor:cleanup}
\end{proof}

\begin{lemma}\label{lem:rsa-is-sticky}
    $\rsa$, $\rsjl$, and $\rsst$ are sticky.
\end{lemma}
\begin{proof}
    $\rrew$ is sticky (\cref{obs:rewriting-preserves-skicky}). Note that $\rnf$ is sticky as well --- rules of $\rnf$ are rules of $\rrew$ with their bodies with cores, thus the rules of $\rnf$ contain fewer join variables. Therefore $\rnf$ is sticky. Finally, note that every subset of a sticky ruleset is sticky as well. As $\rsjl, \rsst \subseteq \rsa \subseteq \rnf$ the lemma holds.
\end{proof}



\subsection*{From $\rs$ to $\rsp$ -- Heavy Lifting}
\newcommand{\ferns}{\mathbb{F}}
\newcommand{\fern}{\mathcal{F}}
\newcommand{\fernbase}{rew(\fern)}
\newcommand{\rsf}{\rs_{\ferns}}

\newcommand{\jlterms}{\mathcal{T}_0}
\newcommand{\stterms}{\mathcal{T}_1}

In this section, we finally delve into the challenging part of the proof. This requires a quick overview of the next few steps. We intend to simplify the ruleset, obtaining $\rsp$, making it relatively straightforward to demonstrate its finite controllability. Let's begin by defining two sets of terms:
%
\begin{align*}
    \jlterms &= \adom{\chase{\dbp, \rsjl}}\\
    \stterms &= \adom{\chase{\dbp, \rsa}} \setminus \jlterms
\end{align*}
\begin{comment}
In the first part of this section we argue that the chase $\chase{\dbp, \rsa}$ is of the following shape:
\begin{figure}[H]
\centering
\includegraphics[width=0.85\linewidth]{figures/R_1.pdf}
\caption{Visualization of the domain of the chase $\chase{\dbp, \rsa}$.}\label{fig:automaton-example}
\end{figure}
\end{comment}
Imagine - noting that $\chase{\chase{\dbp, \rsjl}, \rsa}$ equals $\chase{\dbp, \rsa}$ - that we first run the $\rsjl$ rules over $\dbp$, and then over the resulting instance, the entire $\rsa$. It turns out that there are no atoms in the chase that contain only terms of $\stterms$. This is due to the stickiness of $\rsa$ - non-joinless rules have to propagate join variables to their heads, effectively forcing propagation of $\jlterms$ terms to atoms containing at least one $\stterms$.

\begin{observation}\label{obs:sticky-term-implies-joinless}
    For every atom $\alpha$ of $\chase{\dbp, \rsa}$ if $\alpha$ contains a term of $\stterms$ then it contains a term $\jlterms$ on an $\rsa$-marked position.
\end{observation}
\begin{proof}
    Let $\inst = \chase{\dbp, \rsjl}$. Note that $\chase{\inst, \rsa} = \chase{\dbp, \rsa}$ since $\rsjl \subseteq \rsa$. During the first step of $\chase{\inst, \rsa}$, no joinless rule was fired (as $\inst$ is saturated under $\rsjl$). Therefore, as $\rsa$ is sticky and each rule of $\rsst$ has at least one join variable, every atom produced in $\step{1}{\inst, \rsa}$ contains at least one term of $\jlterms$ in a marked position. After this point, every rule needs to map to at least one of the atoms produced during $\chase{\inst, \rsa}$; therefore, by a straightforward inductive argument, we complete the proof. 
\end{proof}

Of course this means, that any binary atom containing a $\stterms$ term contains at most one:

\begin{corollary}
    No binary atom of $\chase{\dbp, \rsa}$ can contain two $\stterms$ terms.
\end{corollary}
\begin{proof}
    Directly from \cref{obs:sticky-term-implies-joinless}.
\end{proof}

Moreover, we can derive the following strong property regarding binary atoms of $\chase{\dbp, \rsa}$:
\begin{observation}\label{obs:cannot-join-binary-on-sticky-terms}
    Let $\alpha(t_0, t_1)$ and $\beta(s_0, t_1)$ be two atoms of $\chase{\dbp, \rsa}$ such that $t_0, s_0 \in \jlterms$ and $t_1 \in \stterms$ then $t_0 = s_0$. 
\end{observation}
\begin{proof}
    Assume w.l.o.g. that $\alpha$ was derived before $\beta$ during the chase. Therefore, $\beta$ was created by a Datalog rule. From \cref{obs:sticky-term-implies-joinless} we know that $t_0$ appears on an $\rsa$-marked position in $\alpha$. From this we conclude that $t_0$ needs to appear in $\beta$, as $\rsa$ is sticky, and thus $t_0 = s_0$.
\end{proof}

This means we can classify the binary atoms of $\chase{\dbp, \rsa}$ into three categories: 1) atoms forming shallow trees residing between $\mathcal{T}_0$ and $\mathcal{T}_1$, 2) atoms created by $\rsjl$ which use only terms of $\mathcal{T}_0$, and 3) the Datalog atoms of $\rsst$ which contain only terms of $\mathcal{T}_0$. The immediate plan is to remove the non-Datalog part of $\rsst$, one that contributes only to the creation of shallow trees, and replace it with $\rsf$ -- a new ruleset that is far easier to control.



\begin{definition}[Ferns]
A {\em fern} is a rooted poly-tree\footnote{Poly-tree is any instance over binary signature that contains no simple cycle of length at least three when direction of its atoms is disregarded.} of depth $1$ that is a core. Let the set of all ferns be denoted with $\ferns$. Given a fern $\fern$, a {\em fern query} $\fern(x)$ is a CQ obtained from $\fern$ by a bijective replacement of its terms with variables. In this transformation, the root term is replaced by $x$, and all its variables except $x$ are existentially quantified. Given a fern $\fern$ a {\em fern base} $\fernbase$ is the rewriting of $\fern(x)$  against $\rsa$. Let $\rsf$ be the following ruleset:
$$\bigcup_{\fern \in \ferns} \set{\forall{\vy}\; \alpha(x, \vy) \to \fern(x) \mid \exists{\vy}\; \alpha(x, \vy) \in \fernbase}.$$
\end{definition}
Note that a fern can be viewed as a tree, thus by {\em collection of ferns} we mean a {\em forest of trees that are ferns}. 

\begin{observation}\label{obs:rsf-is-stellar}
Every rule of $\rsf$ contains at most one join variable. \orange{Moreover, if 
%a rule of $\rsf$ 
it has a join variable, then it is its only frontier variable.}% $x$.
\end{observation}
\begin{proof}
\blue{Expand this properly.}
Follows from \cref{as:no-intra-atom-joins} \rebut{and stickiness of $\rsa$}.
\end{proof}


\blue{----------------------\\BELOW IS OLD STUFF!!!\\-------------------}

\blue{This is perhaps redundant}
\begin{lemma}\label{lem:after-join-alny-ferns}
Let $\mathcal{B}$ be the set of binary atoms of $\chase{\dbp, \rsa}$ connecting elements of $\jlterms$ and $\stterms$ then $\mathcal{B}$ is a collection of ferns.
\end{lemma}
\begin{proof}
Directly from \cref{obs:cannot-join-binary-on-sticky-terms}
\end{proof}

\blue{This is perhaps redundant}
\begin{observation}\label{obs:no-atoms-with-only-sticky-terms}
The set of atoms $\chase{\dbp, \rsa}|_{\stterms}$ is empty. 
\end{observation}
\begin{proof}
Directly from \cref{obs:sticky-term-implies-joinless}
\end{proof}


\begin{definition}
Let $\rsste$ be the non-Datalog subset of $\rsst$. 
\end{definition}

\begin{lemma}\label{cor:sticky-rsp-equiv}
\rebut{For every Boolean RPQ $\rpq$ we have:} 
\begin{align*}
&\chase{\dbp, \rsa} \models \rpq \iff\\ \iff &\chase{\dbp, \rsa \setminus \rsste \cup \rsf} \models \rpq.
\end{align*}
\end{lemma}
\begin{proof}
From \cref{lem:after-join-alny-ferns,obs:no-atoms-with-only-sticky-terms}.
\end{proof}

Finally, we are able to define $\rsp$ and show that it satisfies one of the required by \cref{lem:sticky-co-semi-decision} properties (\cref{cor:rsp-good-for-entailment}).
\begin{definition}
Let $\rsp$ denote $\rsa \setminus \rsste \cup \rsf$.
\end{definition}

\begin{corollary}\label{cor:rsp-good-for-entailment}
\rebut{For every Boolean RPQ $\rpq$ we have:} 
$$\chase{\dbp, \rs} \models \rpq \iff \chase{\dbp, \rsp} \models \rpq.$$
\end{corollary}
\begin{proof}
    From \cref{lem:rsa-good-entailment} and \cref{cor:sticky-rsp-equiv}.
\end{proof}

Having this, in order to show \cref{lem:sticky-co-semi-decision} and therefore \cref{thm:sticky-main}, we only need to argue that $\rsp$ is $RPQ$-finitely controllable.


\subsection*{Countermodel construction}

In this section we \rebut{build a tool-set necessary to construct finite $RPQ$-countermodels} %$\mathcal{M}$ 
of $\dbp$ and $\rsp$. To this end, we define two equivalence relations over terms of $\chase{\dbp, \rsp}$ and then take the quotient of the chase. As in every such a construction, we have to maintain two properties while constructing the required finite structure. First, that it is a model, and second, that is does not entail the given query. The modelhood is preserved thanks to \emph{stellar types}, while avoiding the entailment of the $RPQ$ is achieved with \emph{regular types}.

\smallskip
\noindent
\orange{\textbf{Stellar types.}}
A {\em stellar query} \orange{(SQ)} is \orange{a} CQ $S(y)$ such that $y$ is the only join variable of $S$ and each atom of $S$ has at most one occurrence of $y$. Given a term $t$ of some instance $\inst$ the {\em stellar type} $\bigstar(t)$ of $t$ is the maximal (up to equivalence) \orange{SQ} $S(y)$ such that $\inst \models S(t)$. A {\em stellar rule} is any existential rule of the following form $$\Forall{\vx}\;\narule{\alpha(\vx, y)}{\vz}{\beta(y, \vz)}$$ \orange{for} $\Exists{\vx}\;\alpha(\vx, y)$ \orange{an SQ}. A ruleset consisting of stellar rules is stellar.

\begin{corollary}\label{cor:rsf-is-stellar}
$\rsf$ is stellar.\quad \orange{\normalfont(From \cref{obs:rsf-is-stellar})}
\end{corollary}

\begin{observation}\label{obs:reminder-is-stellar}
$\rsp \setminus (\rsf \cup \rsjl)$ is stellar.
\end{observation}
\begin{proof}
By the definition the ruleset in question is Datalog, and contains rules with at most a single join-variable.
\end{proof}

Below, for any instance $\inst$ and two of its terms $t$, $t'$ whenever we write $\inst[t,t' \mapsto t'']$ we mean a structure that is obtained from $\inst$ by replacing each occurrence of $t$ and $t'$ with a fresh null $t''$.

\begin{lemma}\label{lem:stellar-id-joinless}
Given two terms $t, t'$ of some instance $\inst$, and a joinless rule $\rho$ it holds:\orange{\quad $\inst \;\models\; \rho \quad\Rightarrow\quad \inst[t,t'\mapsto t''] \;\models\; \rho.$}
\end{lemma}
\begin{proof}
Note, as $\rho$ is joinless, identification of terms does not create new active triggers.
\end{proof}

\begin{lemma}\label{lem:stellar-id-stellar}
Given two terms $t, t'$ of some instance $\inst$ such that $\bigstar(t) = \bigstar(t')$, and a stellar rule $\rho$ it holds: 
$$\inst \;\models\; \rho \quad\Rightarrow\quad \inst[t,t'\mapsto t''] \;\models\; \rho.$$
\end{lemma}
\begin{proof}
Observe that $\bigstar(t'') = \bigstar(t') = \bigstar(t)$ and that the stellar types of other terms do not change after identification ($\heartsuit$). Let $\alpha(\vx)$ be a head of $\rho$, with $\vx$ being a tuple of its frontier variables. Note that as $\rho$ is stellar $\vx$ consists of a single variable. Thus, due to ($\heartsuit$) satisfaction of $\alpha(\vx)$ is preserved $\inst'$.
\end{proof}

\begin{comment}
The following is quite specific but it describes necessary property of the remainder of $\rsp$
\orange{
\begin{lemma}\label{lem:stellar-id-sticky}
Given two terms $t, t'$ of some instance $\inst$ such that $\bigstar(t) = \bigstar(t')$, and a single-join, sticky, Datalog, and binary-head rule $\rho$ it holds: 
$$\inst \;\models\; \rho \quad\Rightarrow\quad \inst, t = t' \;\models\; \rho.$$
\end{lemma}
\begin{proof}
Easy and tedious.
\end{proof}
}
\end{comment}

\begin{corollary}\label{cor:stellar-types-id}
Given two terms $t, t'$ of some instance $\inst$ such that $\bigstar(t) = \bigstar(t')$ it holds:\orange{\quad
$\inst \models \rsp \quad\Rightarrow\quad \inst[t,t'\mapsto t''] \models \rsp.$}
\end{corollary}
\begin{proof}
\orange{From \cref{cor:rsf-is-stellar}, Obs. \ref{obs:reminder-is-stellar}, \cref{lem:stellar-id-joinless}, and \ref{lem:stellar-id-stellar}.}
\end{proof}



\newcommand{\regtyp}{\hspace{0.4mm}\updownarrow\hspace{-0.4mm}}
%\smallskip
\noindent
\orange{\textbf{Regular types.}}
Given an DFA $\autom = \pair{\states, \Sigma, \delta, \state_0, \state_{\mathrm{fin}}}$, two its states $\state, \state' \in \states$, an instance $\inst$, and one of its terms $t$, we write $\state \to \state'(t)$ ($\state \leftarrow \state'(t)$) \iffi there exists a term $t'$ of $\inst$ and a path from $t'$ to $t$ (from $t$ to $t'$) labelled with a word $w$ such that $\delta^*(\state, w) = \state'$. Define the {\em regular type} $\regtyp(t)$ of $t$ as the set of above-defined expressions holding for $t$ that $t$ satisfies w.r.t $\inst$ and $\autom$. 


\begin{lemma}\label{lem:regular-types-id}
    Given a Boolean RPQ $\rpq$ and a DFA $\autom$ defining it, an instance $\inst$, and two of its terms $t$ and $t'$ such that $\regtyp(t) = \regtyp(t')$. Then:
    $$\inst \models \rpq \quad\iff\quad \inst[t,t'\mapsto t''] \models \rpq.$$
\end{lemma}
\begin{proof}
Note that the regular types are present in both $\inst$ and $\inst[t,t'\mapsto t'']$ are the same. \orange{Note,} that for any instance $\jnst$ we have $\jnst \models \rpq$ \iffi there exists a term $s$ of $\jnst$ \orange{satisfying} $\state_0 \to \state_{\mathrm{fin}} (s)$.
\end{proof}

Note that such defined regular types indeed work for any instance, and therefore this part of the countermodel construction is independent from $\rs$ and $\rsp$. 


\subsection*{Finish line}
\begin{corollary}\label{cor:rsp-fin-cont}
The ruleset $\rsp$ is finitely RPQ-controllable.
\end{corollary}
\begin{proof}
Assume $\chase{\dbp, \rsp} \not\models \rpq$ for some \rebut{Boolean} RPQ $\rpq$.
Let $\mathcal{M}$ be a structure obtained from $\chase{\dbp, \rsp}$ by identifying terms that are of the same stellar and regular type. 

From \cref{cor:stellar-types-id,lem:regular-types-id} we have that $\mathcal{M}$ is a model of $\dbp$ and $\rsp$ but not of $\rpq$.  
As there is finite number of both the stellar and regular types the model $\mathcal{M}$ is finite. 
\end{proof}

\noindent
This and Cor.~\ref{cor:sticky-rsp-equiv} grant us \cref{lem:sticky-co-semi-decision} which gives us \cref{thm:sticky-main}.


==> x4a-alternate-decidable.tex <==
\section{Decidablility of regular path queries over sticky rulesets}

In the next section we are going to show the proof of the following:

\begin{theorem}\label{thm:sticky-main}
RPQ entailment under sticky rulesets is decidable.
\end{theorem}


To simplify the quite involved proof of the above we restrict the query language to RPQs. However, it is straightforward to obtain the following as a consequence:

\begin{theorem}\label{thm:extended-sticky-main}
2RPQ entailment under sticky rulesets is decidable.
\end{theorem}

One can obtain \cref{thm:extended-sticky-main} by a simple reduction. Take a sticky ruleset $\rs$ over signature $\sig$, a database $\db$ and a 2RPQ $\rpq$. Keep $\db$ intact, add a single rule 
    ${\epred(x,y)}\to{{\epred'}(y,x)}$
to $\rs$ for every binary predicate $\epred \in \sig$, and replace every occurence of inverted symbol $\inv{\epred}$ with \rebut{$\epred'$} in the regular expression of $\rpq$. 
%
It should be clear that entailment questions for original and transformed problems are equivalent. Finally, note that the transformation preserves stickiness of the ruleset. 


%\section{Proof of Theorem~\ref{thm:sticky-main}}\label{sec:sticky-main-proof}

The rest of the section is dedicated to the proof of \Cref{thm:sticky-main}. 
\textbf{\textit{Fix, until the end of this section, a database $\db$, a sticky ruleset $\rs$.}}
%and a RPQ $\rpq$. 
We show decidability through two semi-decision procedures.

\rebut{
\noindent
\textbf{On repeated free variables of RPQs.} We would like to note that, by definition, we do not support RPQs of the form $A(x,x)$ and $\exists{x}.A(x,x)$. It appears to us that handling any "variable joining" requires a very distinct set of techniques. Therefore, we feel that those two cases should naturally fall under class of \emph{conjunctive} (2)RPQs. This should become apparent in the following section.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RECURSIVE ENUMERABILITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recursive Enumerability}
This part \rebut{follows standard technique appealing to recursive enumerability of consequences of FO theories}.

\begin{observation}
Given a Boolean RPQ $Q = \Exists{x,y} A(x,y)$ one can write a Datalog rule set $\rs_Q$ with one distinguished nullary predicate \textsc{Goal}, such that for every instance \rebut{$\db$}:
$$\database,\; \ruleset \models Q \quad\iff\quad \database,\; \rebut{\ruleset \,\cup\,} \rs_Q \models \textsc{Goal}.$$ 
\end{observation}
\begin{proof}
Let $\autom$ be any DFA with its regular language being the same as the language of $A$. For every state $q_i$ of $\autom$ let $\qpred_i$ be a \rebut{fresh} and corresponding \rebut{unary} relational symbol. Then the Datalog rule set $\rs_Q$ contains the following rules:
\begin{align*}
\adrule{}{\qpred_{0}(x)} \tag{for the starting state $q_0$}\\
\adrule{\qpred_{i}(x), \epred(x,y)}{\qpred_{j}(y)} \tag{if $\pair{q_i, \epred} \mapsto q_j$ is in $\autom$}\\
\adrule{\qpred_{f}(x)}{\textsc{Goal}}\tag{for the accepting state $q_f$}
\end{align*}
%
In essence, the chase of any instance and the above ruleset will have every domain element annotated with the states in which they can be reached by a walking automaton starting from some other domain element.
\end{proof}

From this, as $\db \wedge \rs \wedge \rs_{\rpq}$ is an FO theory, we can semi-decide $\db, \rs \cup \rs_{\rpq} \models \textsc{Goal}$. Thus, we can semi-decide $\db, \rs \models \rpq$ as well.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CO RECURSIVE STUFF and PROMISE OF R+ and D+
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Co-recursive Enumerability}
This part is much harder than the above and requiring a fresh approach. 
In essence, the co-procedure exploits the fact that, after a certain pre-processing of $\db$ and $\rs$, non-entailment of \rebut{any} $\rpq$ is witnessed by a finite instance.

\begin{definition}\label{def:finite-controllability}
Given a query language $\mathfrak{L}$ and a ruleset $\rs$ we say that $\rs$ is {\em finitely $\mathfrak{L}$-controllable} \iffi for every $Q \in \mathfrak{L}$ and for every database $\db$ such that $\db, \rs \not\models Q$ there exists a finite model $\mathcal{M}$ of $\db$ and $\rs$ such that $\mathcal{M} \not\models Q$.
\end{definition} 

\begin{lemma}\label{lem:sticky-co-semi-decision}
One can compute a database $\dbp$ and a ruleset $\rsp$ such that $\rsp$ is finitely RPQ-controllable \rebut{and such that for every Boolean RPQ $\rpq$ we have}  $\db, \rs \models \rpq \;\iff\; \dbp, \rsp \models \rpq$.
\end{lemma}

In view of this lemma, we can ``co-semidecide'' $\db, \rs \models \rpq$ (that is, semi-decide $\db, \rs \not\models \rpq$) 
by enumerating all finite instances and terminating whenever a $\rpq$-countermodel of $\dbp, \rsp$ is found.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HOW TO PROVE THE ABOVE PROMISE SPLIT THE PROOF INTO FC AND REDUCING TO STELLAR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overview of the proof of \cref{lem:sticky-co-semi-decision}}

Before we could start discussing the proof, let us introduce a specific class of rulesets:

\smallskip
\noindent
\orange{\textbf{Stellar rules.}}
A {\em stellar query} \orange{(SQ)} is \orange{a} CQ $S(y)$ such that $y$ is the only join variable of $S$ and each atom of $S$ has at most one occurrence of $y$. A {\em stellar rule} is any existential rule of the following form $$\Forall{\vx}\;\narule{\alpha(\vx, y)}{\vz}{\beta(y, \vz)}$$ \orange{for} $\Exists{\vx}\;\alpha(\vx, y)$ \orange{an SQ}. A ruleset consisting of stellar rules is \emph{stellar}.

Our goal is to construct $\dbp, \rsp$ in such a way that $\rsp$ consists only of stellar and joinless rules and that $\dbp, \rsp$ entail exactly the same Boolean RPQs as $\db, \rs$. The reason behind this is as follows:

\begin{lemma}\label{lem:stellar-joinless-are-fc}
    Any ruleset consisting of stellar and joinless rules is $RPQ$-finitely controllable.
\end{lemma}

We first show how to prove the above lemma, and then show the construction of required $\rsp$ and $\dbp$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FINITE CONTROLLABILITY FOR JOINLESS AND STELLAR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{finite $RPQ$-controllability}
\newcommand{\rss}{\mathcal{S}}
Assume $\rss$ is a ruleset consisting of a number of stellar and joinless rules.
To prove its finite $RPQ$-controllability, we present, given some database and an RPQ that is not entailed, a construction of a finite countermodel. This construction involves two key aspects: the "finite model" aspect and the "counter" (non-entailment) aspect. We begin with the first.

For any instance $\inst$ and two of its terms $t$, $t'$ we denote with $\inst[t,t' \mapsto t'']$ a structure obtained from $\inst$ by replacing each occurrence of $t$ and $t'$ with a fresh null $t''$. 

Keeping modelhood of a ``folded'' structure for joinless rules is trivial:

\begin{observation}\label{obs:modelhood-for-joinless}
    For a joinless rule $\rho$, an instance $\inst$ s.t. $\inst \models \rho$, and terms $s,t$ of $\inst$ we have: $\inst[s,t \mapsto u] \models \rho$. 
\end{observation}
\begin{proof}
    Note, as $\rho$ is joinless, identification of terms could not create new active triggers.
\end{proof}

For stellar rules, however, we need to define an kind of an 1-type that allows modelhood-preserving identification of terms with the same type. To this end, we define:

%-----------------------------------------------------------------------------
% STELLAR TYPES
%-----------------------------------------------------------------------------
\smallskip
\noindent
\orange{\textbf{Stellar types.}}
Given a term $t$ of some instance $\inst$ the {\em stellar type} $\bigstar(t)$ of $t$ is the maximal (up to equivalence) \orange{SQ} $S(y)$ such that $\inst \models S(t)$.

\begin{observation}\label{obs:modelhood-for-stellar}
 For a stellar rule $\rho$, an instance $\inst$ such that $\inst \models \rho$, and terms $s,t$ of $\inst$ such that $\bigstar(s) = \bigstar(t)$ we have: $\inst[s,t \mapsto u] \models \rho$.
\end{observation}
\begin{proof}
Observe that $\bigstar(s) = \bigstar(t) = \bigstar(u)$ and that the stellar types of other terms do not change after identification ($\heartsuit$). Let $\alpha(\vx)$ be a head of $\rho$, with $\vx$ being a tuple of its frontier variables. Note that as $\rho$ is stellar $\vx$ consists of a single variable. Thus, due to ($\heartsuit$) satisfaction of $\alpha(\vx)$ is preserved.
\end{proof}

\begin{corollary}\label{cor:preserving-modelhood-for-s}
For an instance $\inst$ such that $\inst \models \rss$, and terms $s,t$ of $\inst$ such that $\bigstar(s) = \bigstar(t)$ we have: $\inst[s,t \mapsto u] \models \rss$.
\end{corollary}
\begin{proof}
Directly from Observations~\ref{obs:modelhood-for-joinless}~and~\ref{obs:modelhood-for-stellar}.
\end{proof}

The following takes care of the ``counter'' part of the finite countermodel construction. Note that the following is independent from $\rs$ and $\rsp$. 

%-----------------------------------------------------------------------------
% REGULAR TYPES
%-----------------------------------------------------------------------------
\newcommand{\regtyp}{\hspace{0.4mm}\updownarrow\hspace{-0.4mm}}
%\smallskip
\noindent
\orange{\textbf{Regular types.}}
Given an DFA $\autom = \pair{\states, \Sigma, \delta, \state_0, \state_{\mathrm{fin}}}$, two its states $\state, \state' \in \states$, an instance $\inst$, and one of its terms $t$, we write $\state \to \state'(t)$ ($\state \leftarrow \state'(t)$) \iffi there exists a term $t'$ of $\inst$ and a path from $t'$ to $t$ (from $t$ to $t'$) labelled with a word $w$ such that $\delta^*(\state, w) = \state'$. Define the {\em regular type} $\regtyp(t)$ of $t$ as the set of above-defined expressions holding for $t$ that $t$ satisfies w.r.t $\inst$ and $\autom$. 


\begin{lemma}\label{lem:regular-types-id}
    Given a Boolean RPQ $\rpq$ and a DFA $\autom$ defining it, an instance $\inst$, and two of its terms $t$ and $t'$ such that $\regtyp(t) = \regtyp(t')$. Then:
    $$\inst \models \rpq \quad\iff\quad \inst[t,t'\mapsto t''] \models \rpq.$$
\end{lemma}
\begin{proof}
Note that the regular types are present in both $\inst$ and $\inst[t,t'\mapsto t'']$ are the same. \orange{Note,} that for any instance $\jnst$ we have $\jnst \models \rpq$ \iffi there exists a term $s$ of $\jnst$ \orange{satisfying} $\state_0 \to \state_{\mathrm{fin}} (s)$.
\end{proof}

%-----------------------------------------------------------------------------
% FINAL FINITE CONT. ARGUMENT
%-----------------------------------------------------------------------------


We are now ready to demonstrate that $\rss$ is finitely $RPQ$-controllable. Let $\db'$ be any database and $Q$ be any Boolean $RPQ$. Suppose $\chase{\db', \rss} \not\models Q$. Let $\inst$ be an instance obtained from $\chase{\db', \rss}$ by identifying all nulls that share the same regular and stellar types. With the support of \cref{cor:preserving-modelhood-for-s} and \cref{lem:regular-types-id}, considering that there are only finitely many stellar and regular types for $Q$, we conclude that $\inst$ is finite, acts as a model of $\db'$ and $\rss$, and does not entail $Q$. Thus, we establish \cref{lem:stellar-joinless-are-fc}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  CONSTRUCTION OF D+ and R+
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Construction of $\dbp$ and $\rsp$}
\blue{TODO better subsections subsubsections choice}
In this section we shall construct $\dbp$ and $\rsp$ satisfying the two following lemmas, and thus, using \cref{lem:stellar-joinless-are-fc}, satisfy the requirements of \cref{lem:sticky-co-semi-decision}.

\begin{lemma}\label{lem:rsp-is-stellar-and-joinless}
    $\rsp$ consists of joinless and stellar rules.
\end{lemma}

%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% EQUIVALENCE LEMMA WITH MULTIPLE IN-BETWEEN STEPS
\begin{lemma}\label{lem:dbp-rsp-equiv-db-rs}
    For every Boolean query $Q$ it holds:
    $$\chase{\db, \rs}\models Q \iff \chase{\dbp, \rsp} \models Q.$$
\end{lemma}

In order to obtain the first of the two lemmas, we perform a couple of surgeries on the initially fixed sticky ruleset $\rs$. As we progress, at each point, we maintain multiple in-between variants of the second lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ASSERTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection*{Streamlining the presentation}
For the sake of the presentation, we make the following assertion. It streamlines the presentation of the proof, and could be achieved by taking equivalent but cosmetically transformed databases, rulesets, and RPQs instead of the provided ones.
\begin{assertion}\label{as:no-intra-atom-joins}
Every database and ruleset contains no atom with repeated terms.
\end{assertion} 
We defer the precise definition of such transformation to the \cref{app:transformation} and below we present a high-level overview.
We preprocess $\db$ and $\rs$ by annotating their atoms. For example, $\epred(a, b, b, c)$ becomes $\epred_{1,2,2,3}(a,b,c)$. Rulesets have to be expanded by taking every potential equivalence relation on body variables into account while applying the same transformation to their heads. For example:
$\narule{\epred(x,y)}{z}{\rpred(x, y, z, z)}$ s expanded into:
\begin{align*}
\arule{\epred_{1,2}(x,y)}{z}{\rpred_{1,2,3,3}(x, y, z)},\\ \arule{\epred_{1,1}(x)}{z}{\rpred_{1,1,2,2}(x,z)}
\end{align*}
A careful reader will notice this transformation necessitates slight adjustment of the definition of $RPQs$. That is, RPQs should be allowed to ``read'' unary predicates of the form $\epred_{1,1}$ as ones representing binary loops $\epred$. 

As said before, the above assertion is meant to avoid adding yet another layer of transformations to the already complicated proof that follows. It is straightforward to verify that various ruleset-surgeries performed after this point do not invalidate the above assertion in the slightest.



%=============================================================================
% Rewritting-away non-stellar rules
%=============================================================================
\subsubsection*{Rewriting-away non-stellar rules}
Here, we heavily rely on both the stickiness (and thus {\fus}ness) of $\rs$. The below relies on the idea that for the \fus rulesets, rewriting can be also applied to bodies of rules -- yielding a new equivalent ruleset. This transformation preserves stickiness of the input ruleset and, importantly, it preserves Boolean RPQ entailment.

\newcommand{\rewop}{\mathtt{rew}}
\newcommand{\rrew}{\rew(\rs)}
\newcommand{\rhorew}{\rew(\rho, \rs)}
\begin{definition}\label{def:body-rewriting}
For a rule $\rho \in \rs$ of the form:~$\cnarule{\alpha(\vx, \vy)}{\vz}{\beta(\vy, \vz)}$
let $\rhorew$ be the following set of existential rules:
\begin{align*}
    &\set{\narule{\gamma(\vx', \vy)}{\vz}{\beta(\vy, \vz) \mid \\ &(\Exists{\vx'}\gamma(\vx', \vy)) \;\in\; \rew(\Exists{\vx} \alpha(\vx, \vy), \rs)}}.
\end{align*} 
%
Finally, let $\rrew= \rs \cup \bigcup_{\rho \in \rs}\; \rhorew.$
\end{definition}

\begin{lemma}\label{obs:rewriting-preserves-skicky}
The ruleset $\rrew$ is sticky.
\end{lemma}
\begin{proof}
\rebut{Can be found in} \cref{sec:rewriting-preserves-skicky}.
\end{proof}

%-----------------------------------------------------------------------------
% Quickness
%-----------------------------------------------------------------------------


We are now ready to present the main tool of the construction. The idea behind it can be traced back to \cite{journey-paper}.

\begin{definition}\label{def:quick}
\orange{A ruleset} $\rs'$ is {\em quick} \iffi for every instance $\inst$ and every atom $\beta$ of $\chase{\inst, \rs'}$ it holds that if all frontier terms of $\beta$ are contained in $\adom{\inst}$ then $\beta \in \step{1}{\inst, \rs'}$.
\end{definition}

The technique of quickening, is quite powerful. It allows simplification of rulesets as well as general streamlining of proof-related reasoning. We have that:

\begin{lemma}\label{lem:frontier}
$\rrew$ is quick.
\end{lemma}
\begin{proof}
Let $\beta(\vt, \vs) \in \chase{\inst, \rrew}$ and let $\vt$ denote the frontier terms of $\beta$. Assume that $\vt$ is contained in $\inst$ but $\beta$ is not.

Let $\rho$ be the rule that created $\beta$ during the chase and let it be of the following, general form:\orange{
$\;\narule{\alpha(\vx, \vy)}{\vz}{\beta(\vy, \vz)}.\;$}
From the above, note that $\inst, \rrew \models \Exists{\vx}\alpha(\vx, \vt)$.

If $\rho \in \rs$ then there exists $\gamma(\vx', \vy)$ such that: 
$(\Exists{\vx'}\gamma(\vx', \vy)) \in \rew(\Exists{\vx} \alpha(\vx, \vy), \rs)$ and
$\inst \models \Exists{\vx'}\gamma(\vx', \vt)$. Therefore, from definition of $\rrew$, there exists a rule $\rho' \in \rrew$ (with $\gamma$ begin its body) such that $\rho'$ derives $\beta$ in $\step{1}{\inst, \rs'}$.

If $\rho \not\in \rs$ then let $\rho'$ be such that $\rho \in \rew(\rho', \rs)$ and $\rho' \in \rs$. As $\rho \in \rew(\rho', \rs)$  we know that $\rho'$ can be used as well during the chase to obtain $\beta$. Thus, we can use the above reasoning for $\rho'$ instead of $\rho$ to complete the proof of the lemma.
\end{proof}


%-----------------------------------------------------------------------------
% INTRODUCING RNF
%-----------------------------------------------------------------------------
The ruleset we have ($\rrew$) is almost the one we need to construct $\rsp$. As we work with sticky rulesets, we are generally focused on variable joins appearing in rules. The idea behind, the following step of the proof can be explained using the following simple CQ $\Phi(x) = \Exists{y, y'}\epred(x,y),\epred(x,y')$. Note that the variable join on $x$ is not necessary to express $\Phi$ as it is equivalent to its core $\Phi'(x) = \Exists{y} \epred(x,y)$. Therefore:

\begin{definition}\label{def:rnf}
Let $\rnf$ be $\set{\core(\rho) \mid \rho \in \rrew}$.
\end{definition}

As taking cores of bodies of rules produces an equivalent ruleset we have:

\begin{observation}\label{lem:rnf-good}
    $\chase{\db, \rnf} = \chase{\db, \rrew}$, and $\rnf$ is both sticky and quick.
\end{observation}

%-----------------------------------------------------------------------------
% Final step R+ and D+
%-----------------------------------------------------------------------------

Now we are ready to introduce $\rsp$. Surprisingly, we only have to do the following:

\begin{definition}
    Let $\rsp$ be $\rnf$ with all rules having two joins removed.
\end{definition}

This is almost perfect. Unfortunately, a few binary atoms are lost.

\begin{lemma}
    $\chase{\db, \rsp}$ and $\chase{\db, \rnf}$ when restricted to binary atoms containing at least one Skolem term are equal.
\end{lemma}
\begin{proof}
    \blue{TODO}
\end{proof}

Note that in the above, the only binary atoms that are missing are those which $\rnf$ derives over database constants. There is a simple solution to that problem, let:

\begin{definition}
Let $\dbp = \chase{\db, \rnf}|_{\adom{\db}}$
\end{definition}

\cref{lem:sticky-co-semi-decision} requires that $\dbp$ is computable. As $\rnf$ is sticky and therefore \fus it is the case.

\begin{observation}\label{obs:dbp-is-computable}
$\dbp$ is computable. \blue{Remember to ref it!}
\end{observation}
\begin{proof}
As $\rnf$ is \fus we can rewrite every atomic query and ask if it holds for any tuple of constants of $\db$.
\end{proof}

\begin{corollary}
For every Boolean $RPQ$ $Q$
    $\chase{\db, \rnf} \models Q \iff \chase{\dbp, \rsp} \models Q.$
\end{corollary}

Moreover, by the definition of $\rsp$ we have:
\begin{corollary}
    The ruleset $\rsp$ is stellar.
\end{corollary}


\begin{comment}

\blue{----------------------------------------------\\}
\blue{--------------- BELOW IS OLD, ----------------\\}
\blue{----------------------------------------------\\}

%-----------------------------------------------------------------------------
% INTRODUCING RSA
%-----------------------------------------------------------------------------

\newcommand{\rsa}{\rs_\mathrm{pruned}}
\newcommand{\rsjl}{\rs_\mathrm{joinless}}
\newcommand{\rsst}{\rs_\mathrm{sticky}}
\newcommand{\rsste}{\rs_\mathrm{sticky}^{\exists}}

We are now ready to remove a subset of Datalog rules from $\rnf$. As it turns out, the remainder of Datalog is stellar or joinless. Let $\rs'$ be the subset of $\rnf$ that contains Datalog rules having two or more distinct join variables, and let $\rsa$ denote $\rnf \setminus \rs'$. Then we have:

\begin{observation}\label{obs:rsa-datalog-is-stellar-or-joinless}
    Every Datalog rule of $\rsa$ is stellar or joinless.
\end{observation}
\begin{proof}
    Let $\rho$ be a Datalog rule of $\rsa$ that is not joinless. By definition $\rho$ has at most one join variable. Note $\rsa$ is sticky, as it is a subset of $\rnf$ which is sticky (\cref{lem:rnf-is-sticky}). Therefore, the only join variable of $\rho$ - there can be no others in $\rho$ by definition of $\rsa$ - is its frontier variable. Thus $\rho$ is stellar.
\end{proof}

%-----------------------------------------------------------------------------
% INTRODUCING D+
%-----------------------------------------------------------------------------
The transformation step resulting in $\rsa$ is no longer Boolean $RPQ$ entailment preserving under $\db$. However, it is enough to use an extension of $\db$ that is fully saturated under $\rs$.

\begin{definition}
Let $\dbp = \chase{\db, \rs}|_{\adom{\db}}$
\end{definition}

\cref{lem:sticky-co-semi-decision} requires that $\dbp$ is computable. As $\rs$ is sticky and therefore \fus it is the case.

\begin{observation}\label{obs:dbp-is-computable}
$\dbp$ is computable. \blue{Remember to ref it!}
\end{observation}
\begin{proof}
As $\rs$ is \fus we can rewrite every atomic query and ask if it holds for any tuple of constants of $\db$.
\end{proof}

The following is the next intermediate step of \cref{lem:dbp-rsp-equiv-db-rs}.

\begin{lemma}\label{lem:rsa-is-equiv-db-rs}
For every Boolean $RPQ$ $Q$ we have 
$$\chase{\db, \rnf} \models Q \iff  \chase{\dbp, \rsa} \models Q.$$
\end{lemma}
\begin{proof}
\blue{TODO FIX IT A BIT!}
\rebut{Can be found in \cref{app:cor:cleanup}}
\end{proof}

Note that the above might be a bit counter-intuitive as it seems we remove important bits of the ruleset. To some degree it is the case, as given any database $\db'$ it might not be true that $\chase{\db', \rnf} = \chase{\db', \rnf \setminus \rs'}$. However, the crucial aspect is that we focus solely on $\dbp$, which is already saturated in Datalog.

Introduction of $\rsa$, and both \cref{obs:rsa-datalog-is-stellar-or-joinless} and \cref{lem:rsa-is-equiv-db-rs} marks an important milestone in the proof. In order to use \cref{lem:stellar-joinless-are-fc}, however, we still have to take care of the subset of $\rsa$ that is at the same time non-joinless, non-stellar, and non-Datalog. 


%=============================================================================
% REMOVING STICKY EXISTENTIAL PART - THIS IS OLD HEAVY LIFTING
%=============================================================================
\subsubsection*{Final transformation to $\rsp$}
\newcommand{\ferns}{\mathbb{F}}
\newcommand{\fern}{\mathcal{F}}
\newcommand{\fernbase}{rew(\fern)}
\newcommand{\rsf}{\rs_{\ferns}}

\newcommand{\jlterms}{\mathcal{T}_0}
\newcommand{\stterms}{\mathcal{T}_1}

Let $\rsjl$ be the joinless subset of $\rsa$ and let $\rsst$ be its remainder. Clearly, each of those rulesets is sticky, as they are all subsets of $\rnf$ which is  sticky (\cref{lem:rnf-is-sticky}). Let:
%
\begin{align*}
    \jlterms &= \adom{\chase{\dbp, \rsjl}}\\
    \stterms &= \adom{\chase{\dbp, \rsa}} \setminus \jlterms
\end{align*}
\end{comment}
\begin{comment}
In the first part of this section we argue that the chase $\chase{\dbp, \rsa}$ is of the following shape:
\begin{figure}[H]
\centering
\includegraphics[width=0.85\linewidth]{figures/R_1.pdf}
\caption{Visualization of the domain of the chase $\chase{\dbp, \rsa}$.}\label{fig:automaton-example}
\end{figure}
\end{comment}
\begin{comment}
Let us discuss the above two sets of terms. Imagine - noting that $\chase{\chase{\dbp, \rsjl}, \rsa}$ equals $\chase{\dbp, \rsa}$ - that we first run the $\rsjl$ rules over $\dbp$, and then over the resulting instance, the entire $\rsa$. It turns out that there are no atoms in the chase that contain only terms of $\stterms$. This is due to the stickiness of $\rsa$ - non-joinless rules have to propagate join variables to their heads, effectively forcing propagation of $\jlterms$ terms to atoms containing at least one $\stterms$.


\begin{observation}\label{obs:sticky-term-implies-joinless}
    For every atom $\alpha$ of $\chase{\dbp, \rsa}$ if $\alpha$ contains a term of $\stterms$ then it contains a term $\jlterms$ on an $\rsa$-marked position.
\end{observation}
\begin{proof}
    Let $\inst = \chase{\dbp, \rsjl}$. Note that $\chase{\inst, \rsa} = \chase{\dbp, \rsa}$ since $\rsjl \subseteq \rsa$. During the first step of $\chase{\inst, \rsa}$, no joinless rule was fired (as $\inst$ is saturated under $\rsjl$). Therefore, as $\rsa$ is sticky and each rule of $\rsst$ has at least one join variable, every atom produced in $\step{1}{\inst, \rsa}$ contains at least one term of $\jlterms$ in a marked position. After this point, every rule needs to map to at least one of the atoms produced during $\chase{\inst, \rsa}$; therefore, by a straightforward inductive argument, we complete the proof. 
\end{proof}

Of course this means, that any binary atom containing a $\stterms$ term contains at most one:

\begin{corollary}
    No binary atom of $\chase{\dbp, \rsa}$ can contain two $\stterms$ terms.
\end{corollary}
\begin{proof}
    Directly from \cref{obs:sticky-term-implies-joinless}.
\end{proof}

Moreover, we can derive the following strong property regarding binary atoms of $\chase{\dbp, \rsa}$:
\begin{observation}\label{obs:cannot-join-binary-on-sticky-terms}
    Let $\alpha(t_0, t_1)$ and $\beta(s_0, t_1)$ be two atoms of $\chase{\dbp, \rsa}$ such that $t_0, s_0 \in \jlterms$ and $t_1 \in \stterms$ then $t_0 = s_0$. 
\end{observation}
\begin{proof}
    Assume w.l.o.g. that $\alpha$ was derived before $\beta$ during the chase. Therefore, $\beta$ was created by a Datalog rule. From \cref{obs:sticky-term-implies-joinless} we know that $t_0$ appears on an $\rsa$-marked position in $\alpha$. From this we conclude that $t_0$ needs to appear in $\beta$, as $\rsa$ is sticky, and thus $t_0 = s_0$.
\end{proof}

This means we can classify the binary atoms of $\chase{\dbp, \rsa}$ into three categories: 1) atoms forming shallow trees residing between $\mathcal{T}_0$ and $\mathcal{T}_1$, 2) atoms created by $\rsjl$ which use only terms of $\mathcal{T}_0$, and 3) the Datalog atoms of $\rsst$ which contain only terms of $\mathcal{T}_0$. We argue now, that no atom of the first kind can use a non-stellar rule in its derivation.

\begin{definition}
    Let $\rsp$ be $\rsa$ with all its non-stellar, non-joinless, and non-Datalog rules removed. 
\end{definition}

The following is straightforward by definition of $\rsa$ and $\rsp$.
\begin{observation}
    $\rsp$ consists of only joinless and stellar rules.
\end{observation}
\begin{proof}
    By definition $\rsa$ does not contain non-stellar and non-joinless rules.  
\end{proof}

\begin{lemma}
    When constrained to binary atoms $\chase{\dbp, \rsa}$ and $\chase{\dbp, \rsp}$ are equal.
\end{lemma}
\begin{proof}
    Note that $\chase{\dbp, \rsp} \subseteq \chase{\dbp, \rsa}$ as $\rsp \subseteq \rsa$. Take any binary atom $\alpha(s,t)$ of $\chase{\dbp, \rsa}$. We shall show that $\alpha(s,t) \in \chase{\dbp, \rsp}$. We first argue that if $\alpha$ is of the second of third kind then $\alpha \in \chase{\dbp, \rsa}$. If $\alpha$ is of the second kind it simply is an element of $\chase{\dbp, \rsjl}$ 
\end{proof}


\blue{TODO tomorrow:
\begin{itemize}
    \item We can just remove rules that have two joins altogether. Cross positions in atoms created by rules having two joins. No Quick binary Datalog rule is going to use doubly crossed atoms it in it's derivation tree, because it connects immediately to an existential atom which do not crosses its existential term. Moreover, no existential rule (quickness is not used here) can use doubly crossed atoms in its derivation tree, because sticky. From this we can simply remove all two-join rules from the quick ruleset and be done with it. The proof serves as a testament to the quickness technique.
    \item Stellar = only one join variable and it is a frontier variable consider allowing zero join vriables
    \item Fix stellar argument in FC argument
    \item perhaps we can remove doubly joined rules completely after we have quickenss?
    \item The proof of the above should go like this. Stuff wholly contained in $T_0$ cannot use atoms created after a double join - this requires quickness.
\end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THIS IS SEMI-OLD STUF, IF WE DO NOT NEED FERNS AND CAN ARGUE, THAT NON-STELLAR PARTS CANNOT CONTRIBUTE TO CREATION OF BINARY ATOMS, WE DO NOT NEED THAT STEP THAT MUCH.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{definition}[Ferns]
A {\em fern} is a rooted poly-tree\footnote{Poly-tree is any instance over binary signature that contains no simple cycle of length at least three when direction of its atoms is disregarded.} of depth $1$ that is a core. Let the set of all ferns be denoted with $\ferns$. Given a fern $\fern$, a {\em fern query} $\fern(x)$ is a CQ obtained from $\fern$ by a bijective replacement of its terms with variables. In this transformation, the root term is replaced by $x$, and all its variables except $x$ are existentially quantified. Given a fern $\fern$ a {\em fern base} $\fernbase$ is the rewriting of $\fern(x)$  against $\rsa$. Let $\rsf$ be the following ruleset:
$$\bigcup_{\fern \in \ferns} \set{\forall{\vy}\; \alpha(x, \vy) \to \fern(x) \mid \exists{\vy}\; \alpha(x, \vy) \in \fernbase}.$$
\noindent
Note that a fern can be viewed as a tree, thus by {\em collection of ferns} we mean a {\em forest of trees that are ferns}. 
\end{definition}

\begin{definition}
Let
Let $\rsste$ be the non-Datalog subset of $\rsst$. And let $\rsp$ be $\rsa \setminus \rsste \cup \rsf$.
\end{definition}


\begin{lemma}\label{lem:rsp-dbp-equiv-rsa-dbp}
\rebut{For every Boolean RPQ $\rpq$ we have:} 
\begin{align*}
&\chase{\dbp, \rsa} \models \rpq \iff\\ \iff &\chase{\dbp, \rsp} \models \rpq.
\end{align*}
\end{lemma}
\begin{proof}
Can be found in the \cref{}
From \cref{lem:after-join-alny-ferns,obs:no-atoms-with-only-sticky-terms}.
\end{proof}


\blue{This is perhaps redundant}
\begin{lemma}\label{lem:after-join-alny-ferns}
Let $\mathcal{B}$ be the set of binary atoms of $\chase{\dbp, \rsa}$ connecting elements of $\jlterms$ and $\stterms$ then $\mathcal{B}$ is a collection of ferns.
\end{lemma}
\begin{proof}
Directly from \cref{obs:cannot-join-binary-on-sticky-terms}
\end{proof}

\blue{This is perhaps redundant}
\begin{observation}\label{obs:no-atoms-with-only-sticky-terms}
The set of atoms $\chase{\dbp, \rsa}|_{\stterms}$ is empty. 
\end{observation}
\begin{proof}
Directly from \cref{obs:sticky-term-implies-joinless}
\end{proof}





Finally, we are able to define $\rsp$ and show that it satisfies one of the required by \cref{lem:sticky-co-semi-decision} properties (\cref{cor:rsp-good-for-entailment}).
\begin{definition}
Let $\rsp$ denote $\rsa \setminus \rsste \cup \rsf$.
\end{definition}

\begin{corollary}\label{cor:rsp-good-for-entailment}
\rebut{For every Boolean RPQ $\rpq$ we have:} 
$$\chase{\dbp, \rs} \models \rpq \iff \chase{\dbp, \rsp} \models \rpq.$$
\end{corollary}
\begin{proof}
    From \cref{lem:rsa-good-entailment} and \cref{cor:sticky-rsp-equiv}.
\end{proof}

Having this, in order to show \cref{lem:sticky-co-semi-decision} and therefore \cref{thm:sticky-main}, we only need to argue that $\rsp$ is $RPQ$-finitely controllable.




\begin{observation}\label{obs:rsf-is-stellar}
Every rule of $\rsf$ contains at most one join variable. \orange{Moreover, if 
%a rule of $\rsf$ 
it has a join variable, then it is its only frontier variable.}% $x$.
\end{observation}
\begin{proof}
\blue{Expand this properly.}
Follows from \cref{as:no-intra-atom-joins} \rebut{and stickiness of $\rsa$}.
\end{proof}
\end{comment}
